Real-time Deformation with Coupled Cages and Skeletons

Skeleton-based and cage-based deformation techniques represent the two most popular approaches to control real-time deformations of digital shapes and are, to a vast extent, complementary to one another. Despite their complementary roles, high-end modeling packages do not allow for seamless integration of such control structures, thus inducing a considerable burden on the user to maintain them synchronized. In this paper, we propose a framework that seamlessly combines rigging skeletons and deformation cages, granting artists with a real-time deformation system that operates using any smooth combination of the two approaches. By coupling the deformation spaces of cages and skeletons, we access a much larger space, containing poses that are impossible to obtain by acting solely on a skeleton or a cage. Our method is oblivious to the specific techniques used to perform skinning and cage-based deformation, securing it compatible with pre-existing tools. We demonstrate the usefulness of our hybrid approach on a variety of examples.

==> 025_scenario.tex <==
% !TEX root = 00_main.tex

\section{Scenario}
\label{sec:scenario}

\enrico{This part is verbose and talks too much of animation. Content would be better moved to the Introduction.}

Our project is intended to support the animators in performing their work of posing and refining the characters.

The usual input to the deformation step of the pipeline is a mesh, representing the detailed description of the character, its rigging skeleton, usually composed by a standard number of bones, and a cage framing the mesh.
The mesh and the skeleton are linked through the skinning weights, and the mesh and the cages are connected using barycentric coordinates on the cages' vertices.
There are, typically, no connections between the skeleton and the cage.
The character is posed in the base pose, also known as rest pose or t-pose.
The artist works on several different poses of the mesh using its skeleton: the deformation acts as a set of rotations of the skeleton's joints that are connected in a hierarchical graph to keep the whole model consistent.
The mesh follows the movements of the skeleton using the skinning weights that are carefully designed to reproduce natural movements.
The artist could need, anytime during the posing, to modify the mesh, for instance, to simulate hard breathing by the character or to perform unnatural modification required by the script.
Currently, the deformation systems are unable to support an interlaced succession of skeleton-based and cage-based modifications of the characters since, as stated before, these two manipulators are not directly connected.
Using our method, the artist can, instead, have a seamless combination of the two. The proposed method takes care of the update and sync the changes of the cages onto the skeleton and moves the cage according to the change in pose due to the rigging.
In the following, we will explain how we achieved such a smooth integration that, in the end, is entirely transparent to the final user.

